Galaxy formation in the Planck cosmology II. Star formation histories and post-processing magnitude reconstruction

We adapt the L-Galaxies semi-analytic model to follow the star-formation histories (SFH) of galaxies -- by which we mean a record of the formation time and metallicities of the stars that are present in each galaxy at a given time. We use these to construct stellar spectra in post-processing, which offers large efficiency savings and allows user-defined spectral bands and dust models to be applied to data stored in the Millennium data repository. We contrast model SFHs from the Millennium Simulation with observed ones from the VESPA algorithm as applied to the SDSS-7 catalogue. The overall agreement is good, with both simulated and SDSS galaxies showing a steeper SFH with increased stellar mass. The SFHs of blue and red galaxies, however, show poor agreement between data and simulations, which may indicate that the termination of star formation is too abrupt in the models. The mean star-formation rate (SFR) of model galaxies is well-defined and is accurately modelled by a double power law at all redshifts: SFR proportional to $1/(x^{-1.39}+x^{1.33})$, where $x=(t_a-t)/3.0\,$Gyr, $t$ is the age of the stars and $t_a$ is the loopback time to the onset of galaxy formation; above a redshift of unity, this is well approximated by a gamma function: SFR proportional to $x^{1.5}e^{-x}$, where $x=(t_a-t)/2.0\,$Gyr. Individual galaxies, however, show a wide dispersion about this mean. When split by mass, the SFR peaks earlier for high-mass galaxies than for lower-mass ones, and we interpret this downsizing as a mass-dependence in the evolution of the quenched fraction: the SFHs of star-forming galaxies show only a weak mass dependence.

==> disc.tex <==
An understanding of SFHs is important to correctly interpret observations of
galaxies, especially when hgh-resolution spectra are not available.  The effect
of the SFH of a galaxy on the recovered mass and SFR has been investigated by
\citet{PMT12} who show that both the stellar mass and the star-formation rate of
galaxies can be in error by a dex or more if incorrect SFHs are used, and concur
with \citet{MPR10} that an increasing SFR shoudl be adopted at high-redshift.
Similarly, \citet{PKB13} show that the modelling of dust in high-redshift
galaxies can be misinterpretted if steeply-declining SFHs are used and can lead
to erroneous estimated SFRs, and \citet{MHD14} found that the masses of SMGs can
be underestimated under the same circumstances.


==> notes.tex <==
\citet{WDW11} look at the SFHs of 60 nearby dwarf galaxies with a variety of
morphologies.  They find that all formed most of their stars and have had a
nearly constant star-formation rate since, averaged over bins of width of 1\,Gyr
or more.  Only in the last 1\,Gyr do dwarf irregulars show an enhanced
star-formation rate, and this could be a selection effect associated with their
classification.  The masses of these galaxies are much lower than those
investigated in this paper, but the results agree with the trend seen in
\Fig{sfhmass} and \Tab{ssfr} that low-mass galaxies have approximately constant
star-formation rates and low quiescent fractions.
\todo{Actually, that's not true, as we do NOT find a drop in SFR from early
  times.}

\citet{MWC14} claim a massive upturn in SFR for dwarfs as you look back to high
redshift, but I don't believe it as it is all based on making stars 13\,Gyr old
rather than 10\,Gyr -- in other words, a small shift in stellar ages woudl make
the result go away.


==> ppmagapp.tex <==
\section{Post-processing magnitude errors}
\label{app:ppmag}

Table~\ref{tab:ppmag} shows the root-mean-square difference between magnitudes
  calculated on-the-fly during the running of the code (i.e.~using the finest
  possible time resolution) and those calculated in post-processing, using
  different numbers of SFH bins.  Histograms of the distributions of magnitude
  differences, plus a discussion of their origin, can be found in \Sec{ppmag}.

\begin{table*}
\begin{center}
\caption{This table shows the root-mean-square difference between magnitudes
  calculated on-the-fly during the running of the code and those calculated in
  post-processing.}
\label{tab:ppmag}
\begin{tabular}{lcccccc}
\hline
& & without dust  & & & with dust &\\
$z=0$ & \multicolumn{3}{c}{\hrulefill}& \multicolumn{3}{c}{\hrulefill}\\
&$N_\mathrm{max}=1$ &$N_\mathrm{max}=2$
&$N_\mathrm{max}=4$  &$N_\mathrm{max}=1$
&$N_\mathrm{max}=2$ &$N_\mathrm{max}=4$ \\
\hline
GALEX $FUV$               &3.02 &0.29 &0.16 &2.53 &0.38 &0.29 \\
GALEX $NUV$              &1.79 &0.05 &0.03 &1.47 &0.16 &0.16 \\
SDSS $u$                     &0.76 &0.03 &0.01 &0.66 &0.06 &0.05 \\
SDSS $g$                     &0.50 &0.02 &0.00 &0.46 &0.03 &0.02 \\
SDSS $z$                     &0.36 &0.02 &0.00 &0.33 &0.02 &0.02 \\ 
VISTA $J$                     &0.35 &0.02 &0.00 &0.32 &0.02 &0.02 \\ 
VISTA $K_s$                 &0.33 &0.01 &0.01 &0.31 &0.02 &0.02 \\ 
IRAC $3.6_{\mu \rm{m}}$ &0.38 &0.01 &0.00 &0.36 &0.03 &0.02 \\
\hline
& & without dust  & & & with dust &\\
$z=2$ & \multicolumn{3}{c}{\hrulefill}& \multicolumn{3}{c}{\hrulefill}\\
&$N_\mathrm{max}=1$ &$N_\mathrm{max}=2$
&$N_\mathrm{max}=4$  &$N_\mathrm{max}=1$
&$N_\mathrm{max}=2$ &$N_\mathrm{max}=4$ \\
\hline
GALEX $FUV$               &1.74 &0.04 &0.01 &1.14 &0.27 &0.26 \\
GALEX $NUV$              &1.39 &0.02 &0.00 &0.95 &0.21 &0.20 \\
SDSS $u$                     &0.88 &0.02 &0.00 &0.63 &0.13 &0.12 \\
SDSS $g$                     &0.64 &0.01 &0.00 &0.47 &0.09 &0.09 \\
SDSS $z$                     &0.39 &0.01 &0.00 &0.33 &0.04 &0.04 \\ 
VISTA $J$                     &0.33 &0.01 &0.00 &0.30 &0.02 &0.02 \\ 
VISTA $K_s$                 &0.32 &0.01 &0.00 &0.30 &0.01 &0.01 \\ 
IRAC $3.6_{\mu \rm{m}}$ &0.31 &0.01 &0.00 &0.28 &0.02 &0.02 \\
\hline
\end{tabular}
\end{center}
\end{table*}



==> sfhindapp.tex <==
\section{Individual star-formation histories}
\label{app:sfhind}

Ownership: Sorour

\Sec{sfhind}\ showed changes in star-formation rates in fixed intervals of
100\,Myr.  \Fig{sfhindapp} shows instead the ratio of star formation within the
most recent and the second most recent decile of the age of the
Universe at that time.  As can be seen from the right-hand panel, this gives a more
pronounced progression from increasing star-formation rates at high redshift, to
declining ones at $z=0$.

\begin{figure*}
\centering
\includegraphics[width=85mm]{figs/sfhind.ps}
\includegraphics[width=85mm]{figs/sfhindzoom.ps}
\caption{The ratio of the star-formation rate in the most recent 100\,Myr to
  that in the previous 100\,Myr for galaxies at redshift 3 with masses exceeding
  10$^{10.5}$\Msun in the HWT13 model.  The different line-styles refer
to different mass ranges and the vertical lines indicate the 5, 50 \& 95
percentiles of each distribution.  The right-hand panel
shows a zoom in about the centre of the range.  \comment{Note: these are
  currently the same plots as \Fig{sfhind}, acting as placeholders.}} 
\label{fig:sfhindapp}
\end{figure*} 

\todo{Replace these plots with the correct ones.}

